Double Descent Risk and Volume Saturation Effects: A Geometric Perspective

The appearance of the double-descent risk phenomenon has received growing interest in the machine learning and statistics community, as it challenges well-understood notions behind the U-shaped train-test curves. Motivated through Rissanen's minimum description length (MDL), Balasubramanian's Occam's Razor, and Amari's information geometry, we investigate how the logarithm of the model volume: $\log V$, works to extend intuition behind the AIC and BIC model selection criteria. We find that for the particular model classes of isotropic linear regression and statistical lattices, the $\log V$ term may be decomposed into a sum of distinct components, each of which assist in their explanations of the appearance of this phenomenon. In particular they suggest why generalization error does not necessarily continue to grow with increasing model dimensionality.

==> MAIN_Broader_Impact.tex <==
\section*{Broader Impacts}

\textbf{Who are the Beneficiaries of this Research?} The main beneficiaries of this research are theoreticians who are investigating learning theories to better understand (i) The nature of generalization error in highly parameterized regimes, and (ii) The nature of double descent risk. We also anticipate that such research can be used empiricists who are looking to form a better understanding of how their models may work in the highly parameterised regimes.

\textbf{Who is Put at Disadvantage from this Research?} We believe that no one will be \textit{put} at a direct disadvantage of this research per se. However it is possible for a new researcher in this area to \textit{feel} at a disadvantage, as this work serves as an addition to an already large of corpus of existing literature on the subject. Especially as this research is reliant upon information geometry, which is a difficult topic in of itself, this could lengthen the time taken by a new researcher in this field to feel ``up to speed'' in this area. To this end, we have tried to offer as many explanations, and references as possible in order to encourage everyone's intuition.  

\textbf{What are the Consequences of a System Failure?} At this point in time, the work is designed to be used in order to encourage one's understanding of some of the deeper implications of double descent risk, and generalization error. It is possible for some readers to become very reliant on the underlying explanations, which are still a topic under heavy investigation, and so it is possible for the analysis to fail in newer, more exotic statistical models. To this end, if a system is in production, and is built without any empirically driven analysis (and only based on the proposals in this work), we anticipate that the model will not work up to the required standards as intended by the readers, or their workplace. The consequences of this will have ranging severities, as the research is not specific to one context. 

\textbf{Does the Task Leverage any Data Biases?} The experiments in this paper work with data which is randomly generated from an isotropic Gaussian distribution. To this end, our data is naturally free from the biases which may effect other datasets. We've also been careful to ensure that the experiments are reproducible, and easy to understand. Ultimately we believe that this point is not as applicable to us as the others. 


Although this research is centred on theoretical developments, we have outlined some additional ethical considerations which are important to consider for this research. In particular these include: (1) Privacy, (2) Participation, (3) Inclusion \& Inequality, (4) Safety \& Security, and (5) Transparency. The relationship between these are oulined in Figure \ref{fig:ethics}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Images/Ethical_Stack2.PNG}
    \caption{The anticipated ethical mindmap for this research, in order to help clarify areas of potential broader impact.}
    \label{fig:ethics}
\end{figure}

In conclusion, there are evidently various ethical notions which become apparent upon closer inspection of this work. We welcome this work for all to read, and sincerely ask that any inspirations derived from this theoretical analysis are not used for any nefarious purposes, obstructions of justice, and or ethically objectionable activities.
